RiskRAG: A Data-Driven Solution for Improved AI Model Risk Reporting

Risk reporting is essential for documenting AI models, yet only 14% of model cards mention risks, out of which 96% copying content from a small set of cards, leading to a lack of actionable insights. Existing proposals for improving model cards do not resolve these issues. To address this, we introduce RiskRAG, a Retrieval Augmented Generation based risk reporting solution guided by five design requirements we identified from literature, and co-design with 16 developers: identifying diverse model-specific risks, clearly presenting and prioritizing them, contextualizing for real-world uses, and offering actionable mitigation strategies. Drawing from 450K model cards and 600 real-world incidents, RiskRAG pre-populates contextualized risk reports. A preliminary study with 50 developers showed that they preferred RiskRAG over standard model cards, as it better met all the design requirements. A final study with 38 developers, 40 designers, and 37 media professionals showed that RiskRAG improved their way of selecting the AI model for a specific application, encouraging a more careful and deliberative decision-making. The RiskRAG project page is accessible at: https://social-dynamics.net/ai-risks/card.

==> sections/06_Ethics.tex <==
\subsubsection{Ethics}
All three studies, including co-design and evaluation, were approved by the authors' organization. Participants received informed consent detailing the study's purpose, data usage, and their rights. Confidentiality and anonymity were ensured, with data handled according to established ethical guidelines. Participants recruited via Prolific were compensated at GBP 12 per hour. Research materials, such as study artifacts and the thematic analysis codebook, were shared in compliance with transparency criteria outlined by \cite{salehzadehniksiratChangesResearchEthics2023}.
